Data Secrecy in Distributed Storage Systems under Exact Repair

The problem of securing data against eavesdropping in distributed storage systems is studied. The focus is on systems that use linear codes and implement exact repair to recover from node failures.The maximum file size that can be stored securely is determined for systems in which all the available nodes help in repair (i.e., repair degree $d=n-1$, where $n$ is the total number of nodes) and for any number of compromised nodes. Similar results in the literature are restricted to the case of at most two compromised nodes. Moreover, new explicit upper bounds are given on the maximum secure file size for systems with $d<n-1$. The key ingredients for the contribution of this paper are new results on subspace intersection for the data downloaded during repair. The new bounds imply the interesting fact that the maximum data that can be stored securely decreases exponentially with the number of compromised nodes.

==> Arxiv Netcod2013/results.tex <==

%!TEX root = SecureMDS_Netcod2013.tex



\section{Main Results}\label{sec:results}
%State the technical results in the form of theorems, lemmas,É
%proofs will come later.  I will embellish later and explain what the theorems mean. But for now this is important because it will help me explain our contributions in the intro.
In this section, we state our main results. The proofs will follow in Section \ref{sec:proofs} after give a rough idea behind the results in Section \ref{sec:intuition}. The following lemma provides a lower bound on the sum of subspaces\footnote{The sum of subspaces $B$, $C$ is defined as $B+C = \{b+c:b\in B, c\in C\}$.} associated with the repair bandwidth from a particular node, when it aids in the repair of multiple nodes.
\begin{lemma}\label{lem1}
Consider an $(n,k,d)$-DSS in the systematic form with nodes having storage capacity $\alpha$. Let nodes $[k]$ be the systematic nodes and let $V_{i,j}$ be the $\beta \times \alpha$ matrix associated with the exact repair of node $j$ by node $i$. Then, for $d = n-1$ and for each $i \in [k]$, we have
\begin{eqnarray}\label{eq:lem1}
\dim\left(\sum_{j \in {\cal A}}V_{i,j}\right) &\ge& \left(1 - \left(\frac{n-k-1}{n-k}\right)^{|{\cal A}|}\right)\alpha,
\end{eqnarray}
where ${\cal A} \subseteq [k]\backslash \{i\}$ and $V_{i,j}$ is the subspace corresponding to the matrix.
\end{lemma}

\smallskip
The next theorem gives an upper bound on the (linear coding) secrecy capacity $C_s(\alpha)$ for a given number of compromised nodes.
\begin{theorem}\label{thm1}
Consider an $(n,k,d)$-DSS with a node storage capacity of $\alpha$, which stores an optimal bandwidth linear MDS code for exact repair of systematic nodes. Suppose an eavesdropper gains access to the data stored in $\ell_1$ nodes and the data downloaded during the repair of $\ell_2$ systematic nodes, such that
\begin{eqnarray*}
\ell_1 + \ell_2 &<& k.
\end{eqnarray*}
The achievable secure file size $M^s$ for the given MSR code is then upper bounded by
\begin{eqnarray}\label{eq:thm1}
M^{s} &\le& (k-\ell_1-\ell_2)\left(1-\frac{1}{d-k+1}\right)^{\ell_2}\alpha.
\end{eqnarray}
\end{theorem}

\smallskip
The next theorem establishes that the upper bound in Theorem \ref{thm1} is achievable when $d = n-1$.
\begin{theorem}\label{thm2}
For an $(n, k, d)$-DSS with $d = n-1$, the secrecy capacity for optimal bandwidth MDS codes such that any systematic node is exact-repairable using a linear coding, is achievable for $\alpha = (n-k)^k$ and is given by
\begin{eqnarray}
C_s(\alpha) &=& (k-\ell_1-\ell_2)\left(1-\frac{1}{n-k}\right)^{\ell_2}\alpha.
\end{eqnarray}
Moreover, the capacity is achievable for all $(\ell_1, \ell_2)$.
\end{theorem}
\begin{IEEEproof}
The proof follows from \cite[Theorem 10]{RKSV13} which describes an achievability scheme by precoding a ($n,k$) zigzag code \cite{TWB13} using a maximum rank distance code.
\end{IEEEproof}
%{\red
%\begin{theorem}\label{thm3}
%Exactness is not free for secure MDS. Update: turns out this is not true. Or at least we don't know.
%\end{theorem}
%}

==> results.tex <==

%!TEX root = SecureMDS_Netcod2013.tex



\section{Main Results}\label{sec:results}
%State the technical results in the form of theorems, lemmas,É
%proofs will come later.  I will embellish later and explain what the theorems mean. But for now this is important because it will help me explain our contributions in the intro.
In this section, we state our main results. The proofs will follow in Section \ref{sec:proofs} after give a rough idea behind the results in Section \ref{sec:intuition}. The following lemma provides a lower bound on the sum of subspaces\footnote{The sum of subspaces $B$, $C$ is defined as $B+C = \{b+c:b\in B, c\in C\}$.} associated with the repair bandwidth from a particular node, when it aids in the repair of multiple nodes.
\begin{lemma}\label{lem1}
Consider an $(n,k,d)$-DSS in the systematic form with nodes having storage capacity $\alpha$. Let nodes $[k]$ be the systematic nodes and let $V_{i,j}$ be the $\beta \times \alpha$ matrix associated with the exact repair of node $j$ by node $i$. Then, for $d = n-1$ and for each $i \in [k]$, we have
\begin{eqnarray}\label{eq:lem1}
\dim\left(\sum_{j \in {\cal A}}V_{i,j}\right) &\ge& \left(1 - \left(\frac{n-k-1}{n-k}\right)^{|{\cal A}|}\right)\alpha,
\end{eqnarray}
where ${\cal A} \subseteq [k]\backslash \{i\}$ and $V_{i,j}$ is the subspace corresponding to the matrix.
\end{lemma}

\smallskip
The next theorem gives an upper bound on the (linear coding) secrecy capacity $C_s(\alpha)$ for a given number of compromised nodes.
\begin{theorem}\label{thm1}
Consider an $(n,k,d)$-DSS with a node storage capacity of $\alpha$, which stores an optimal bandwidth linear MDS code for exact repair of systematic nodes. Suppose an eavesdropper gains access to the data stored in $\ell_1$ nodes and the data downloaded during the repair of $\ell_2$ systematic nodes, such that
\begin{eqnarray*}
\ell_1 + \ell_2 &<& k.
\end{eqnarray*}
The achievable secure file size $M^s$ for the given MSR code is then upper bounded by
\begin{eqnarray}\label{eq:thm1}
M^{s} &\le& (k-\ell_1-\ell_2)\left(1-\frac{1}{d-k+1}\right)^{\ell_2}\alpha.
\end{eqnarray}
\end{theorem}

\smallskip
The next theorem establishes that the upper bound in Theorem \ref{thm1} is achievable when $d = n-1$.
\begin{theorem}\label{thm2}
For an $(n, k, d)$-DSS with $d = n-1$, the secrecy capacity for optimal bandwidth MDS codes such that any systematic node is exact-repairable using a linear coding, is achievable for $\alpha = (n-k)^k$ and is given by
\begin{eqnarray}
C_s(\alpha) &=& (k-\ell_1-\ell_2)\left(1-\frac{1}{n-k}\right)^{\ell_2}\alpha.
\end{eqnarray}
Moreover, the capacity is achievable for all $(\ell_1, \ell_2)$.
\end{theorem}
\begin{IEEEproof}
The proof follows from \cite[Theorem 10]{RKSV13} which describes an achievability scheme by precoding a ($n,k$) zigzag code \cite{TWB13} using a maximum rank distance code.
\end{IEEEproof}
%{\red
%\begin{theorem}\label{thm3}
%Exactness is not free for secure MDS. Update: turns out this is not true. Or at least we don't know.
%\end{theorem}
%}
